Augmenting Knowledge Graphs for Better Link Prediction

Embedding methods have demonstrated robust performance on the task of link prediction in knowledge graphs, by mostly encoding entity relationships. Recent methods propose to enhance the loss function with a literal-aware term. In this paper, we propose KGA: a knowledge graph augmentation method that incorporates literals in an embedding model without modifying its loss function. KGA discretizes quantity and year values into bins, and chains these bins both horizontally, modeling neighboring values, and vertically, modeling multiple levels of granularity. KGA is scalable and can be used as a pre-processing step for any existing knowledge graph embedding model. Experiments on legacy benchmarks and a new large benchmark, DWD, show that augmenting the knowledge graph with quantities and years is beneficial for predicting both entities and numbers, as KGA outperforms the vanilla models and other relevant baselines. Our ablation studies confirm that both quantities and years contribute to KGA's performance, and that its performance depends on the discretization and binning settings. We make the code, models, and the DWD benchmark publicly available to facilitate reproducibility and future research.

==> attic/intro.tex <==
\section{Introduction}
\label{sec:intro}

Hyperrelational knowledge graphs (KGs), like Wikidata~\cite{vrandevcic2014wikidata}, represent their knowledge in the form of statements~\cite{galkin2020message}. Each statement consists of a triple, enriched with key-value qualifiers and with references that support its veracity. The statements represent either a relationship between two entities, or provide a literal value (date, quantity, or string) attributed to an entity. Nearly half of the statements in Wikidata are entity relationships, whereas the rest is largely comprised of strings, quantities, and dates.\footnote{\url{https://wikidata-todo.toolforge.org/stats.php}, accessed on Sep 1, 2021} Intuitively, literals and related entities complement each other to form a more comprehensive representation of an entity.

Considering the sparsity and the inherent incompleteness of knowledge graphs, the task of link prediction has been very popular. According to a recent survey~\cite{wang2021survey}, the wide palette of approaches proposed for this task can be mostly classified as either: matrix factorization/decomposition~\cite{chang2014typed}, path-based methods~\cite{lao2011random,grover2016node2vec}, or embedding based methods~\cite{bordes2013translating,trouillon2016complex,yang2014embedding,nickel2011three}. Curiously, all of these methods have repeatedly focused on performing link prediction by only considering Qnode values, i.e., relationship between two entities. The literals attributed to the entities in a knowledge graph are usually ignored, despite them carrying useful information. For instance, a person's date of birth or a company's founding year could contextualize the prediction task to a specific time period of relevance. Similarly, the population of a country represents an implicit information about how big that country is. Analogous to recent work that proposed to enhance link prediction performance by preserving qualifier information~\cite{galkin2020message,rosso2020beyond}, we argue that information encoded in quantity and year literals should be considered by link prediction methods. 

In fact, several efforts incorporate numeric literals into KG embeddings, either by adding a literal-aware term to the scoring function~\cite{garcia2017kblrn,kristiadi2019incorporating}, or by modifying the loss function of the base model in order to balance capturing the KG structure and numeric literals~\cite{wu2018knowledge,tay2017multi,feng2019marine}. These methods leverage the knowledge encoded in literals in order to improve link prediction performance, but they introduce additional parameters and model-specific clauses, which limits their scalability, generalizability to other embedding models, and it might distort the original distribution of the statements in the graph.

In this paper, we propose \textsc{\textit{KGA}}: a knowledge graph augmentation method to incorporate literals for any embedding-based model without modifying its loss function. We focus on embedding-based methods, as these have been shown to be superior over matrix factorization and path-based methods~\cite{lu2020utilizing}. Our contributions are:

\begin{enumerate}
    \item We propose \textsc{\textit{KGA}}: a method for incorporating quantity and year literals into KGs, by chaining the literals vertically, for different granularities of discretization, and horizontally, for neighboring values to each granularity level. KGA is scalable and can be used as a pre-processing step for any existing knowledge graph embedding model. In addition, the discretized bins represent numeric ranges which correspond to the human's approximate comprehension and categorization of numbers~\cite{dehaene2011number}.\footnote{For instance, humans understand that large mountains have thousands of meters of elevation, but it is uncommon to know that Mount Everest has an elevation of 8,848 metres.} %The enriched graph can be used as input to any embedding model, without introducing additional complexity.
    \item We propose a new link prediction benchmark, DWD, which is orders of magnitude larger than existing link prediction datasets, and includes quantities and years. This addresses a notable bottleneck in link prediction, where existing benchmarks are fairly small and have been repeatedly used for evaluating systems in the past, risking overfitting.% many years already.
    \item Both on DWD and on legacy benchmarks, we show that KGA is able to consistently improve performance of various embedding-based link prediction methods, and outperform the baselines. At the same time, it is able to scale to Wikidata's size of more than billion statements, adding only a small overhead to the training time. The ablation studies confirm that both quantities and years contribute to the performance of KGA, and reveal that adding binning depth has a minor impact on the performance. %binning strategies lead to similar 
    \item We show that incorporating literal information also improves the models' performance on predicting quantities and years. Further experiments reveal that the level of binning has a small, yet consistent, impact on the results, and that attributes with more complex value distributions benefit more from fine-grained binning.
    % \item We perform ablation studies in order to confirm our findings. We also analyze the impact of different discretization and organization strategies, observing that a relatively optimal number of bins can be automatically determined per property based on the property value distribution.
    \item We release the entire code, resulting models, and the DWD benchmark, in order to facilitate future research.
\end{enumerate}



% The method discretizes quantity and year values into bins, and chains these bins both horizontally, modeling neighboring values, and vertically, modeling multiple levels of granularity. This method is scalable and can be used as a pre-processing step for any existing knowledge graph embedding model. In addition, the discretized bins correspond to numeric ranges which correspond to the human's approximate comprehension and categorization of numbers~\cite{dehaene2011number}. For instance, we understand that large mountains have thousands of meters of elevation, but it is uncommon to know that Mount Everest has an elevation of 8,848 metres. \filip{more detail about the approach needed}
% We conduct experiments to inspect the impact of enriching the graph on predicting quantities and years, observing constant improvement over the original embeddings and other relevant baselines. We show that incorporating quantities and years has also a consistent positive impact on link prediction, where the task is to predict missing entity relationships. We provide ablation studies to rule out alternative explanations, and show the impact of different discretization strategies and augmentation levels. Besides evaluating on legacy datasets, for fair comparison to prior work, we also devise orders of magnitude larger and natural benchmark for link prediction over Wikidata, which we call DWD. We will release the entire code, resulting models, and the DWD benchmark, in order to facilitate future research.






% \filip{emphasize that producing ranges is a strength of our paper}


% Quantities and dates are useful for link prediction 

% But are generally ignored!

% 1. Improve link prediction by incorporating quantities \& dates

% 2. Do link prediction of quantities \& dates

% 3. Improve performance of all embedding methods

% 4. Scale to Wikidata size

